Check-N-Run: A Checkpointing System for Training Deep Learning Recommendation Models

Checkpoints play an important role in training long running machine learning (ML) models. Checkpoints take a snapshot of an ML model and store it in a non-volatile memory so that they can be used to recover from failures to ensure rapid training progress. In addition, they are used for online training to improve inference prediction accuracy with continuous learning. Given the large and ever increasing model sizes, checkpoint frequency is often bottlenecked by the storage write bandwidth and capacity. When checkpoints are maintained on remote storage, as is the case with many industrial settings, they are also bottlenecked by network bandwidth. We present Check-N-Run, a scalable checkpointing system for training large ML models at Facebook. While Check-N-Run is applicable to long running ML jobs, we focus on checkpointing recommendation models which are currently the largest ML models with Terabytes of model size. Check-N-Run uses two primary techniques to address the size and bandwidth challenges. First, it applies incremental checkpointing, which tracks and checkpoints the modified part of the model. Incremental checkpointing is particularly valuable in the context of recommendation models where only a fraction of the model (stored as embedding tables) is updated on each iteration. Second, Check-N-Run leverages quantization techniques to significantly reduce the checkpoint size, without degrading training accuracy. These techniques allow Check-N-Run to reduce the required write bandwidth by 6-17x and the required capacity by 2.5-8x on real-world models at Facebook, and thereby significantly improve checkpoint capabilities while reducing the total cost of ownership.

==> implementation.tex <==
For incremental checkpointing using the GPU memory training records, the GPU trainer threads update a bit vector associated with each embedding table entry that is updated. This bit vector is used as a mask to determine which entries of the table are modified during the training process and shipped to the CPU and eventually incrementally checkpointing them.

For the sake of simplicity, we track the training records during the forward pass as most of the training records accessed in the forward pass are modified during the backward pass. As tracking training records needs to be done for every batch of records, we implemented it efficiently on the GPU. To hide this tracking overhead, we scheduled this tracking during the all to all communication phase in the backward pass to utilize the GPU idle cycles. We observe a tracking overhead of $\approx1\%$, which we believe is acceptable to us and did not work further on optimizing the tracking implementation. We also investigated this tracking mechanism on CPU, to utilize the CPU idle cycles and use GPU only for making progress in training. However, we observed that the CPU could not keep up with tracking records as fetched for training.

The CPU-based checkpointing threads perform different operations depending on the type of checkpointing option selected. For quantization they perform the appropriate quantization to reduce the size before transferring the checkpoint to the remote storage. For incremental checkpoint they manage the \textit{meta-index} storage to identify which entries in a table are modified and update the structure appropriately. 
